Empty Commitments: When Agents Promise What They Cannot Deliver

A chatbot that says "I will remind you tomorrow" will not run again until the user writes. We call such a promise an empty commitment: a promise of action after the current turn that nothing in the agent's tools or runtime can carry out. Unlike a broken promise, its emptiness is decided by the agent's configuration at the moment of speaking, so it can be detected from a single turn, before deployment or at run time. We define empty commitments on top of commitment semantics, with three failure types, an anchoring condition for promises that a tool could make real, and an outcome taxonomy that separates these failures from honest deferrals and from over-refusal. We build a checker (a setup-blind detector, deterministic feasibility rules, and a response judge) validated against 400 human labels. On a controlled benchmark of 293 follow-up requests across five setups that add one persistence affordance at a time, four open-weight models of 8-14B parameters fail on 45.9% of responses when no tool exists and nothing is stated. A frontier model fails on 4.4%, but it gets there by deferring and asking, not by using the tools it has: promises made without the enabling call remain in every model. Telling the model its runtime, the cheapest fix, cuts open-weight failures nearly in half where nothing is doable and changes nothing where a scheduler exists; a directive capability card removes most failures at the largest cost in over-refusal; running the checker in the loop and rewriting flagged replies removes more at a smaller cost. Code, prompts, model outputs, and human labels are released.

==> tables/setups.tex <==
\begin{tabular}{@{}lp{0.42\columnwidth}cccc@{}}
\toprule
Setup & Tools & Acts later & Sched. & Mem. & Deleg. \\
\midrule
C0 & none & -- & -- & -- & -- \\
C1 & \texttt{get\_current\_time}, \texttt{calculator}, \texttt{search\_docs}, \texttt{lookup\_account} & -- & -- & -- & -- \\
C2 & \texttt{get\_current\_time}, \texttt{calculator}, \texttt{search\_docs}, \texttt{lookup\_account}, \texttt{schedule\_task}, \texttt{create\_reminder} & sched. & \checkmark & -- & -- \\
C3 & \texttt{get\_current\_time}, \texttt{calculator}, \texttt{search\_docs}, \texttt{lookup\_account}, \texttt{memory\_write}, \texttt{memory\_read} & -- & -- & \checkmark & -- \\
C4 & \texttt{get\_current\_time}, \texttt{calculator}, \texttt{search\_docs}, \texttt{lookup\_account}, \texttt{create\_ticket}, \texttt{escalate\_to\_human} & -- & -- & -- & \checkmark \\
\bottomrule
\end{tabular}

